FunnyNet-W: Multimodal Learning of Funny Moments in Videos in the Wild

Automatically understanding funny moments (i.e., the moments that make people laugh) when watching comedy is challenging, as they relate to various features, such as body language, dialogues and culture. In this paper, we propose FunnyNet-W, a model that relies on cross- and self-attention for visual, audio and text data to predict funny moments in videos. Unlike most methods that rely on ground truth data in the form of subtitles, in this work we exploit modalities that come naturally with videos: (a) video frames as they contain visual information indispensable for scene understanding, (b) audio as it contains higher-level cues associated with funny moments, such as intonation, pitch and pauses and (c) text automatically extracted with a speech-to-text model as it can provide rich information when processed by a Large Language Model. To acquire labels for training, we propose an unsupervised approach that spots and labels funny audio moments. We provide experiments on five datasets: the sitcoms TBBT, MHD, MUStARD, Friends, and the TED talk UR-Funny. Extensive experiments and analysis show that FunnyNet-W successfully exploits visual, auditory and textual cues to identify funny moments, while our findings reveal FunnyNet-W's ability to predict funny moments in the wild. FunnyNet-W sets the new state of the art for funny moment detection with multimodal cues on all datasets with and without using ground truth information.

==> ablation_A_encoder.tex <==
\begin{table}[t]
\centering
\caption{Comparison on using different audio encoders for FunnyNet-W prediction. We report two scenarios: 1) using ground truth texts and 2) using automatically generated texts. 
}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc}
    \toprule
    \multicolumn{5}{c}{Automatically generated text} \\
    \midrule
    \multicolumn{3}{c|}{Modality} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ \cline{1-3}
    A & V & $\text{T}^\text{{a}}$ &  &  \\
    \midrule
    Beats & \multirow{4}{*}{VideoMAE} & \multirow{4}{*}{Llama-2} & 78.2 & 65.1 \\
    CAV &  &  & 87.3 & 83.8 \\
    Byol-v2 &  &  & 87.6 & 84.7 \\
    Byol &  &  & 88.2 & 85.6\\
    \bottomrule
    \end{tabular}%}

	\label{tab:ablation_A_encoder}
\end{table}

==> ablation_T_encoder.tex <==
\begin{table}[t]
\centering
\caption{Comparison on using different text encoders for FunnyNet-W prediction. We report two scenarios: 1) using ground truth texts and 2) using automatically generated texts. 
}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc}
    \toprule
    \multicolumn{5}{c}{Ground truth text} \\
    \midrule
    \multicolumn{3}{c|}{Modality} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ \cline{1-3}
    Audio & Vision & Text &  &  \\
    \midrule
    \multirow{3}{*}{Byol} & \multirow{3}{*}{VideoMAE} & Bert & 87.2 & 83.8 \\
     &  & GPT2 & 88.1 & 85.6 \\
     &  & LlaMa-2 & 89.3 & 86.8 \\
    \midrule
    \multicolumn{5}{c}{Automatically generated text} \\
    \midrule
    \multicolumn{3}{c|}{Modality} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ \cline{1-3}
    Audio & Vision & Text &  &  \\
    \midrule
    \multirow{3}{*}{Byol} & \multirow{3}{*}{VideoMAE} & Bert & 85.3 & 82.3 \\
     &  & GPT2 & 85.2 & 82.3 \\
     &  & LlaMa-2 & 88.2 & 85.6 \\
    \bottomrule
    \end{tabular}
	\label{tab:ablation_T_encoder}
\end{table}

==> ablation_V_encoder.tex <==
\begin{table*}[t]
\begin{minipage}[b]{0.32\textwidth}

\centering
\caption{Ablation of visual encoders on Friends. 
%for FunnyNet-W prediction. We report two scenarios: 1) using ground truth texts and 2) using automatically generated texts. 
}
\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{ccc|cc}
    \toprule
    %\multicolumn{5}{c}{Automatically generated text} \\
    \multicolumn{3}{c|}{\textbf{Modality}} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ %\cline{1-3}
    \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{$\text{T}^\text{{a}}$}   &  &  \\
    \midrule
    \multirow{2}{*}{BYOL-A} & Timesformer & \multirow{2}{*}{Bert} & 84.2 & 80.9 \\
    & VideoMAE &  & 85.3 & 82.3 \\
    \toprule
    \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{$\text{T}^\text{{gt}}$} &  &  \\
    \midrule
    \multirow{2}{*}{BYOL-A} & Timesformer & \multirow{2}{*}{Bert} & 84.9 & 80.8 \\
    & VideoMAE &  & 87.2 & 83.8 \\
    
    
    \bottomrule
    
    \end{tabular}}
    \label{tab:ablation_V_encoder}
\end{minipage}
%
\hfill
\begin{minipage}[b]{0.3\textwidth}
\centering
\caption{Ablation of text encoders on Friends.
}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{ccc|cc}
    \toprule
    \multicolumn{3}{c|}{\textbf{Modality}} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ %\cline{1-3}
    \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{$\text{T}^\text{{a}}$} &  &  \\
    \midrule

     \multirow{3}{*}{BYOL-A} & \multirow{3}{*}{VideoMAE} & Bert & 85.3 & 82.3 \\
     &  & GPT2 & 85.2 & 82.3 \\
     &  & LlaMa-2 & 88.2 & 85.6 \\
     
    \bottomrule
    
    \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{$\text{T}^\text{{gt}}$} & F1 & Acc  \\
    \midrule

    \multirow{3}{*}{BYOL-A} & \multirow{3}{*}{VideoMAE} & Bert & 87.2 & 83.8 \\
     &  & GPT2 & 88.1 & 85.6 \\
     &  & LlaMa-2 & 89.3 & 86.8 \\
     
   
    \bottomrule
    \end{tabular}}
	\label{tab:ablation_T_encoder}
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\textwidth}
\centering
\caption{Ablation of audio encoders on Friends. 
}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{ccc|cc}
    \toprule
    \multicolumn{3}{c|}{\textbf{Modality}} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\ %\cline{1-3}
    \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{$\text{T}^\text{{a}}$} &  &  \\
    \midrule
    BEATS & \multirow{4}{*}{VideoMAE} & \multirow{4}{*}{LlaMa-2} & 78.2 & 65.1 \\
    CAV-MAE &  &  & 87.3 & 83.8 \\
    BYOL-A-v2 &  &  & 87.6 & 84.7 \\
    BYOL-A &  &  & 88.2 & 85.6\\
    \bottomrule
    \end{tabular}}

	\label{tab:ablation_A_encoder}
 
\end{minipage}

\caption*{
\small{A: audio, V: visual frames, $\text{T}^\text{{gt}}$: ground truth text, $\text{T}^\text{{a}}$: automatically generated text (text extracted from speech)}}

\end{table*}


==> ablation_auto_manu.tex <==
\begin{table}[t]
	\caption{\small{
		Ablation study of FunnyNet on Friends. We experiment on both the manually (a) and the automatically (b) labelled test sets. We report Precision (Pre), Recall (Rec), F1 score (F1) and Accuracy (Acc) for audio (A), visual (V) and face (F) modalities \todo{Liu, these results are old (they have face and the numbers do not correspond to the numbers we have. Have you run these?}\liu{I didn't do this experiment, they are from ACCV results.}
    }}
    \begin{subtable}[t]{\columnwidth}
        \centering
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{ccc|cccc}
        \toprule
        \multicolumn{3}{c|}{\textbf{Modalities}} & \multicolumn{4}{c}{\cellcolor{mistyrose}{\textbf{Metrics}}}             \\
        \textbf{A}         & \textbf{V}        & \textbf{F}        & \textbf{Pre}      & \textbf{Rec}      & \textbf{F1}       & \textbf{Acc}    \\ \midrule
        \checkmark         & -        & -        & 71.16    & 75.09    & 73.71    & 66.73  \\
        -         & \checkmark        & -        & 72.57    & 73.23    & 72.93    & 63.44  \\
        -         & -        & \checkmark        & 72.58    & 73.22    & 72.94    & 62.13  \\ \midrule
        \checkmark         & \checkmark        & -        & 80.86    & 87.81    & 84.19    & 81.14  \\
        \checkmark         & -        & \checkmark        & 81.13    & 86.89    & 83.91    & 82.22  \\
        \checkmark         & \checkmark        & \checkmark        & 85.09    & 88.56    & 86.79    & 84.75  \\ \bottomrule
       \end{tabular}}
       \caption{Manual labelling}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{\columnwidth}
        \centering
        \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{ccc|cccc}
        \toprule
        \multicolumn{3}{c|}{\textbf{Modalities}} & \multicolumn{4}{c}{\cellcolor{mistyrose}{\textbf{Metrics}}}             \\
        \textbf{A}         & \textbf{V}        & \textbf{F}        & \textbf{Pre}      & \textbf{Rec}      & \textbf{F1}       & \textbf{Acc}    \\ \midrule
        \checkmark         & -        & -        & 70.23    & 75.87    & 72.94    & 67.80  \\
        -         & \checkmark        & -        & 73.08    & 74.49    & 73.77    & 65.01  \\
        -         & -        & \checkmark        & 74.21    & 74.09    & 74.15    & 64.23  \\ \midrule
        \checkmark         & \checkmark        & -        & 81.11    & 88.20    & 84.51    & 82.19  \\
        \checkmark         & -        & \checkmark        & 81.67    & 87.39    & 84.43    & 82.28  \\
        \checkmark         & \checkmark        & \checkmark        & 86.30    & 89.44    & 87.84    & 85.34  \\ \bottomrule
        \end{tabular}}
        \caption{Automatic labelling}
     \end{subtable}
     \label{tab:ablation_auto_manu}
\end{table}





==> ablation_complexity.tex <==
\begin{table}[t]
\centering
\caption{Comparison to the state of the art of FLOPs count (FLOPs), number of parameters (Params) and inference runtime average (Runtime). We report two versions of model complexity, FunnyNet (V+F+A) and FunnyNet-W (V+F+T) with including pre-trained encoders, and FunnyNet$^b$ and FunnyNet-W$^b$ without including pre-trained encoders. 
}
\begin{small}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|rrr}
    \toprule
    \multirow{ 2}{*}{\textbf{Model}} & \textbf{FLOPs} & \textbf{Params} & \textbf{Runtime} \\ 
     & \textbf{($10^9$)} & \textbf{ ($10^6$)} & (ms) \\ 
    \midrule
    MISA 2020 (V+A+T)~\cite{MISA} & 138.8 & 111.2 & 33.64 \\
    HKT 2021 (V+A+T)~\cite{hasan2021humor} & 7.6 & 16.8 & 25.91 \\
    LaughM 2021 (T)~\cite{laught_machine} & 2.5 & 112.4 & 11.15 \\
    \midrule
   FunnyNet$^b$ & 4.4 & 39.5 & 45.25 \\
    FunnyNet (V+F+A) & 190.9 & 126.9 & 45.25 \\
    FunnyNet-W$^b$ & 3.1 & 29.6 & 30.21 \\
    FunnyNet-W (V+F+T) & 72190 & 70228 & 30.21 \\
    \bottomrule
    \end{tabular}}
\end{small}
	\label{tab:profile_models}
\end{table}

==> ablation_loss.tex <==

\begin{table}[t]
    \caption{Ablation of losses used to train FunnyNet-W.
	}
    \centering
        \begin{small}
    %\resizebox{\linewidth}{!}{
\begin{tabular}{cccc|rr}
\toprule

$L_{\text{cls}}$ & $L_{\text{ss}}$ & $L_{\text{koleo}}$ &  $L_{\text{clip}}$ & F1 & Acc \\
\midrule
\checkmark & -- & -- & -- & 70.9 & 68.0 \\
\checkmark & \checkmark & -- & --  & \textbf{88.2} & \textbf{85.6} \\ 
\checkmark & \checkmark & \checkmark & --  & 86.7 & 84.6 \\ 
\checkmark & \checkmark & -- &\checkmark  & 87.3 & 84.6 \\
\checkmark & \checkmark & \checkmark   & \checkmark  
 & 85.4 & 82.2 \\
 \bottomrule
\end{tabular}%}
\end{small}
\label{tab:loss}
\end{table}

==> ablations_modality_caf.tex <==
\begin{table*}[t]
\begin{minipage}[b]{0.35\textwidth}
\centering
	\caption{
	Ablation of modalities of FunnyNet-W on Friends test set.
	}
    \begin{tabular}{lll|rr}
    \toprule
    \multicolumn{3}{c|}{\textbf{Modality}} & \multirow{2}{*}{F1} & \multirow{2}{*}{Acc} \\
    \cellcolor{mistyrose}{V} & \cellcolor{mistyrose}{A} & \cellcolor{mistyrose}{T} & & \\
    \midrule
     \checkmark & -- & --  & 73.2 & 64.1 \\
    -- & \checkmark & -- & 73.7 & 66.6 \\
    -- & -- & \checkmark & 77.8 & 68.1 \\
    \checkmark & \checkmark & -- & 84.3 & 79.3 \\
    -- & \checkmark & \checkmark & 84.5 & 80.3 \\
    \checkmark & -- & \checkmark & 74.9 & 64.3 \\
    \checkmark & \checkmark & \checkmark & \textbf{88.2} & \textbf{85.6} \\
     \bottomrule
    \end{tabular}
	\label{tab:ablation}

\end{minipage}
\hfill
\begin{minipage}[b]{0.6\textwidth}

\centering
\caption{
   Ablation of CAF of FunnyNet-W on Friends test set. (A: audio, V: visual frames, T: text) }
    \begin{tabular}{cc r@{\hspace{3pt}}r r@{\hspace{3pt}}r r@{\hspace{3pt}}r r@{\hspace{3pt}}r}
    \toprule
    \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{CAF}}}   & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{A+V}}} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{A+T}}} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{V+T}}} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{A+V+T}}} \\
    \textbf{Self} & \textbf{Cross} & F1 & Acc    & F1 & Acc & F1 & Acc & F1 & Acc \\ 
    \midrule
    - & -     & 80.1           & 76.5           & 81.0          & 76.9          & 73.5             & 63.8             & 82.4             & 77.8             \\
    \checkmark & -      & 81.1           & 77.3           & 81.4          & 77.5          & 74.4             & 64.4             & 85.7             & 81.8             \\
    - & \checkmark     & 83.6           & 78.7           & 82.3          & 78.7          & 74.6             & 64.2             & 85.4             & 81.4             \\
    \checkmark & \checkmark      & \textbf{84.3}           & \textbf{79.3}           & \textbf{84.5}           & \textbf{80.3}          & \textbf{74.9}             & \textbf{64.3}             & \textbf{88.2}             & \textbf{85.6}             \\ 
    \midrule
    \multicolumn{2}{c}{MMCA~\cite{cross_attn_2}}      &   83.1         &   78.3         &      83.4     &    79.8       &  73.6     &   63.8           &  87.0     &   84.5           \\
    \multicolumn{2}{c}{CoMMA~\cite{tanCOMMA2021}}      &     83.5       &  78.5    &   83.9    &    \textbf{80.3}   &   74.2    &  64.1           &  87.6    &  85.1           \\
    \bottomrule
    \end{tabular}
	\label{tab:ablation_caf}
	
\end{minipage}
\end{table*}




==> ablations_no_use.tex <==
\begin{table}[t]
    \caption{\todo{}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{6pt}}cc@{}}
    \toprule
    \cellcolor{mistyrose}{Loss} & \multicolumn{3}{c@{\hspace{6pt}}}{\cellcolor{mistyrose}{Encoders}} & \multicolumn{2}{c}{\cellcolor{mistyrose}{Metrics}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-6}
      & Audio & Text & Video & F1 & Acc \\
    \midrule
    CLIP & - & - & - & 00.0 & 00.0 \\
    koleo & - & - & - & 00.0 & 00.0 \\
    - & BYOL-Av2 & - & - & 00.0 & 00.0 \\
    - & CAV-MAE & - & - & 00.0 & 00.0 \\
    - & BEATs & - & - & 00.0 & 00.0 \\
    - & - & BERT & - & 00.0 & 00.0 \\
    - & - & GPT-2 & - & 00.0 & 00.0 \\
    - & - & - & TimeSformer & 00.0 & 00.0 \\
    \midrule
    \textbf{NT-Xent} & \textbf{BYOL-A} & \textbf{LLaMA} & \textbf{VideoMAE} & \textbf{00.0} & \textbf{00.0} \\
    \bottomrule
    \end{tabular}}
\end{table}



==> chatbot.tex <==


\begin{table}[t]
    \caption{Chatbot vs FunnyNet-W.} 
    \centering
        \begin{small}
    \resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc}
\toprule
Prompt engineering & Prompt training & F1 & Accuracy \\
\midrule
\multirow{2}{*}{Generic} & - & 14.5 &	41.8 \\
 & \checkmark & 44.3 & 46.5 \\
\multirow{2}{*}{Specific} & - & 64.1 & 53.2 \\
 & \checkmark & 71.1 & 55.9 \\
\midrule
\multicolumn{2}{c|}{FunnyNet-W (T)} & 77.8 & 68.1 \\
\multicolumn{2}{c|}{FunnyNet-W (A+V+T)} & 88.2 & 85.6 \\
\bottomrule
\end{tabular}}
\end{small}
\label{tab:chatbot}
\end{table}

==> figure9-10.tex <==


\begin{figure*}[t]
\includegraphics[width=\linewidth]
{funny_examples_v2.pdf} 
		\caption{Funny moments in the wild. Three examples from sitcoms, movies, and stand-up with diverse contents, e.g. the sitcom does not have canned laughter, the movie contains dramatic acting performance, and the stand-up is a one-man show without interactions.}
		\label{fig:coolappli1}
\end{figure*}



==> figures7-8.tex <==


\begin{figure}[t]

\centerline{\includegraphics[width=\columnwidth]{fig_attn_liu.pdf} }
		\caption{
		CAF attention maps on the test set of Friends.
		(\textit{a},\textit{b},\textit{c}) Cross Attention between the unified feature $F_{U}$ (coming from all modalities) and audio, vision and text; (\textit{d}) Self Attention on $F_{U}$.
  } 
  
		\label{fig:caf_visual}
\end{figure}



==> laugther_general.tex <==
\begin{table*}[t]
    \centering
    \caption{
    Evaluation of Laughter Detection on Friends.
    We compare five versions of our laughter detector, denoted as `Ours', employing different feature encoders, along with two external audio laughter detectors. 
    The last row corresponds to the actual configuration used in FunnyNet-W.
    }
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l r@{\hspace{7pt}}r@{\hspace{7pt}}r@{\hspace{7pt}}r r r@{\hspace{7pt}}r@{\hspace{7pt}}r r r@{\hspace{7pt}}r@{\hspace{7pt}}r}
    \toprule
    & \multicolumn{4}{c}{\cellcolor{mistyrose}{\textbf{Temporal}}} &  & \multicolumn{3}{c}{\cellcolor{mistyrose}{\textbf{Det} IoU = 0.3}} & & \multicolumn{3}{c}{\cellcolor{mistyrose}{\textbf{Det} IoU = 0.7}} \\
    & Acc & Prec & Rec & F1 & \phantom{abc} & Prec & Rec & F1 & \phantom{abc} & Prec & Rec & F1 \\
    \midrule

    LD~\cite{old_laughter_detector} & 43.6 & 35.7 & \textbf{99.0} & 52.3 & & 25.7 & 22.1 & 23.4 & & 4.0 & 3.7 &	3.8 \\
    
    RLD~\cite{new_laughter_detector} & 74.5 & 58.9 & 62.0 & 59.7 &  & 66.2 & 53.7 & 59.1 & & 18.5 & 15.0 &	16.5 \\
    
    \midrule
    
    Ours Wav2CLIP\cite{wav2clip} & 77.6 & 64.5 & 63.7 & 63.7 & & 91.3 & 61.2 & 73.1 & & 49.7 & 33.5 & 39.9 \\
    
    Ours CAV-MAE\cite{gong2023cavmae}  & 84.3 & 75.4 & 74.2 & 74.6 & & 92.3 & 80.0 & 85.6 & & 52.2 & 45.5 & 48.4 \\
    
    Ours BYOL-A\cite{byol_a} & 86.0 & 76.9 & 79.4 & 77.8 & & 94.6 & 82.3 & \textbf{87.8} & & 54.1 & 47.1 &	50.3 \\
        
    Ours BYOL-A-v2\cite{byola_v2} & 82.1 & 67.7 & \textbf{82.6} & 74.1 & & 92.5 & \textbf{83.5} & 87.6 & & 51.9 & 47.0 & 49.2 \\
    
   Ours BEATs\cite{chen2022beats} & \textbf{86.4} &\textbf{78.4} &{78.3} &\textbf{78.1} &{} &\textbf{95.2} &{81.6} &{87.7} &{} &\textbf{55.1} &\textbf{47.3} &\textbf{50.8} \\
    
    \bottomrule
    \end{tabular}
    %}
    \label{tab:audio_results}
\end{table*}


==> sota_general.tex <==
\begin{table*}[t]

\centering
\caption{
Comparison to the state of the art on five datasets. Modalities used per method A: audio, V: visual frames, $\text{T}^\text{{gt}}$: ground truth text (subtitles or transcript), $\text{T}^\text{{a}}$: automatically generated text (text extracted from speech), F: face.
\\
The column `Wild' signifies the methods that can run \emph{in the wild}, i.e., automatically without requiring ground truth information either for training or for testing. Note, most methods require ground truth labels (mostly in the form of textual subtitles or transcripts) both for training and testing. This is in contrast to FunnyNet-W which can automatically process videos in the wild. 
 \\
 $^{\dagger}$Reproduced results: we use the exact model as in~\cite{laught_machine}, pre-train it on Friends and fine-tune it on the other datasets 
}
		\begin{small}
		\resizebox{\linewidth}{!}{
\begin{tabular}{l c rr crr crr crr crr}
\toprule

\multirow{2}{*}{\textbf{Method / Metrics}} & \multirow{2}{*}{\textbf{Wild}} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{TBBT}}} & \phantom{abc} &  \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{MHD}}} & \phantom{abc} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{MUStARD}}} & \phantom{abc} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{UR-Funny}}} & \phantom{abc} & \multicolumn{2}{c}{\cellcolor{mistyrose}{\textbf{Friends}}} \\
&  & F1          & Acc     & \phantom{abc}   & F1         & Acc     & \phantom{abc}   & F1           & Acc & \phantom{abc}         & F1            & Acc & \phantom{abc}         & F1           & Acc          \\ 
\midrule
Random        &        --            & 46.3        & 50.0 & \phantom{abc}      & 56.1       & 50.9  & \phantom{abc}     & 48.3         & 48.7    & \phantom{abc}     & 50.2          & 50.2  & \phantom{abc}       & 51.0         & 51.0         \\
All positive     & --                & 60.3        & 43.2 & \phantom{abc}      & 75.6       & 60.8 & \phantom{abc}      & 66.7         & 50.0      & \phantom{abc}   & 75.4          & 50.7   & \phantom{abc}      & 66.7         & 50.0         \\
All negative        & --             & 0.0         & 56.8   & \phantom{abc}    & 0.0        & 39.2   & \phantom{abc}    & 0.0          & 50.0   & \phantom{abc}      & 0.0           & 49.3 & \phantom{abc}        & 0.0          & 50.0         \\
MUStARD 2019 (V+A+$\text{T}^\text{{gt}}$)~\cite{mustard}    & --              & -           & -  & \phantom{abc}        & -          & -  & \phantom{abc}        & 71.7         & 71.8    & \phantom{abc}     & -             & -    & \phantom{abc}        & -            & -            \\
MSAM 2021 (V+$\text{T}^\text{{gt}}$)~\cite{humor_data}       & --                & -           & -    & \phantom{abc}      & 81.3       & 72.4    & \phantom{abc}   & -            & -      & \phantom{abc}      & -             & -     & \phantom{abc}       & -            & -            \\
MISA 2020 (V+A+$\text{T}^\text{{gt}}$)~\cite{MISA}     & --                & -           & -    & \phantom{abc}      & -          & -     & \phantom{abc}     & -            & 66.2     & \phantom{abc}   & -             & 69.8     & \phantom{abc}    & -            & -            \\
HKT 2021 (V+A+$\text{T}^\text{{gt}}$)~\cite{hasan2021humor}        & --              & -           & -    & \phantom{abc}      & -          & -  & \phantom{abc}        & -            & 79.4    & \phantom{abc}     & -             & 77.4    & \phantom{abc}     & -            & -            \\
LaughM$^{\dagger}$ 2021 ($\text{T}^\text{{gt}}$)~\cite{laught_machine} & --  & 64.2        & 70.5 & \phantom{abc}      & \textbf{86.5}          & 76.3     & \phantom{abc}     & 68.6            & 68.7  & \phantom{abc}      & 71.9  & 67.6  & \phantom{abc} & 74.7 & 59.8     \\
FunnyNet (V+A+$\text{T}^\text{{gt}}$)   ~\cite{funnynet}     & --          & 73.8        & 75.8    & \phantom{abc}  & 83.4       & 78.6   & \phantom{abc}    & 79.5         & 79.9      & \phantom{abc}   & 84.1          & 79.9    & \phantom{abc}     & 88.2         & 85.8         \\
FunnyNet (V+F+A+$\text{T}^\text{{gt}}$)      ~\cite{funnynet}  & --           & 75.9        & 78.3 & \phantom{abc}      & 85.2       & 79.6 & \phantom{abc}      & 83.2         & 82.0     & \phantom{abc}    & 84.4          & 80.2  & \phantom{abc}       & 88.8         & 86.4         \\ 
\textbf{FunnyNet-W (V+A+$\text{T}^\text{{gt}}$)}     & --        &  \textbf{78.5}     &   \textbf{80.0}  & \phantom{abc}  & 84.6 & \textbf{80.1} & \phantom{abc}    & \textbf{85.9} &  \textbf{84.1}    & \phantom{abc}   & \textbf{84.5} & \textbf{80.2}  & \phantom{abc}     & \textbf{89.3}         & \textbf{86.7}        \\
\midrule
FunnyNet: V+F+A    ~\cite{funnynet}    & \checkmark        & 69.6        & 74.0 & \phantom{abc}     & \textbf{84.0}      & \textbf{79.3}  & \phantom{abc}     & \textbf{81.4} & \textbf{81.0}   & \phantom{abc}     & 83.7 & 78.0  & \phantom{abc}      & 86.8 & 84.8         \\
\textbf{FunnyNet-W: V+A+$\text{T}^\text{{a}}$}     & \checkmark            & \textbf{78.2}        & \textbf{79.1}    & \phantom{abc}  & 83.6       & 78.9   & \phantom{abc}    & 80.1         & \textbf{81.0}      & \phantom{abc}   & \textbf{84.2}          & \textbf{80.3}    & \phantom{abc}     & \textbf{88.2}         & \textbf{85.6}         \\

\bottomrule
\end{tabular}
			}
		\end{small}
	\label{tab:sota1}
\end{table*}



==> text_example.tex <==
\begin{table}[t]
    \caption{\small{\liu{Examples of using Chatbot and FunnyNet-W for funny prediction}
	}}
    \centering
        \begin{small}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{OpenAssistant} & \multicolumn{2}{c}{LlaMa 2} & \multirow{2}{*}{FunnyNet-W} \\
     & w/o PT & w PT & w/o PT & w PT &  \\
    You stay out there and think about what you did! It is a duck. It is a bad duck! & No & No & Yes & No & Yes \\
    If I don't get through, they aren't going to fix my phone for free. We can't let them win. It is us vs. them. Yes! & Yes & No & Yes & No & Yes\\
    I hope it won't be too weird. will it? Rache? No, not at all. & Yes & Yes & Yes & Yes & No\\
    
    \end{tabular}}
\end{small}
\label{tab:text_compare}
\end{table}

==> voice.tex <==


\begin{table}[t]
    \caption{Ablation of synthetic and real voice when training and testing FunnyNet-W on Friends.}

    \centering
        \begin{small}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{cc|cccc}
            \toprule
            \multicolumn{2}{c|}{\multirow{3}{*}{Model}} & \multicolumn{4}{c}{Training voice} \\
            \multicolumn{2}{c|}{} & \multicolumn{2}{c}{synthetic} & \multicolumn{2}{c}{real} \\
            \multicolumn{2}{c|}{} & F1 & Accuracy & F1 & Accuracy \\
            \midrule
            \multirow{2}{*}{Test voice} & synthetic & 65.5 & 67.7 & 68.8 & 66.8 \\
             & real & 83.1 & 79.6 & 88.2 & 85.6 \\
             \bottomrule
            \end{tabular}}
        \end{small}
\label{tab:voice}
\end{table}

